Equal Opportunity and Affirmative Action via Counterfactual Predictions

Machine learning (ML) can automate decision-making by learning to predict decisions from historical data. However, these predictors may inherit discriminatory policies from past decisions and reproduce unfair decisions. In this paper, we propose two algorithms that adjust fitted ML predictors to make them fair. We focus on two legal notions of fairness: (a) providing equal opportunity (EO) to individuals regardless of sensitive attributes and (b) repairing historical disadvantages through affirmative action (AA). More technically, we produce fair EO and AA predictors by positing a causal model and considering counterfactual decisions. We prove that the resulting predictors are theoretically optimal in predictive performance while satisfying fairness. We evaluate the algorithms, and the trade-offs between accuracy and fairness, on datasets about admissions, income, credit and recidivism.

==> img/aa_fig.tex <==
% !TEX root = ../fair_dcf.tex
\begin{adjustbox}{height=4cm}
\begin{tikzpicture}
% \tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1, dashed]
[obs/.style={draw,circle,filled,minimum size=1cm}, latent/.style={draw,circle,minimum size=1cm}]
  % Define nodes
  \node[obs]                               (t1) {$A$};
  \node[obs, left=of t1, xshift=-1.2cm]                               (t2) {$S$};
  \node[obs, below=of t2]            (y) {$Y$};  
  \node[obs, below=of t1]            (yeo) {$\hat{Y}^{eo}$};
  \node[obs, below=of yeo]            (yaa) {$\hat{Y}^{aa}$};
  % Connect the nodes
  \edge {t2} {y, t1} ; 
  \edge {t1} {y, yeo} ;
  \edge {yeo} {yaa};
  \edge {t2} {yaa};

\end{tikzpicture}
\end{adjustbox}

==> preamble/preamble_acronyms.tex <==
% !TEX root = template.tex

\newacronym{KL}{kl}{Kullback-Leibler}
\newacronym{EO}{eo}{equal opportunities}
\newacronym{AA}{aa}{affirmative action}
\newacronym{FTU}{ftu}{fairness through unawareness}
\newacronym{PS}{ps}{personal statement}
\newacronym{SEM}{sem}{structural equation model}
\newacronym{ML}{ml}{machine learning}

\newacronym{CS}{cs}{computer science}


==> preamble/preamble_fix_amslineno.tex <==
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname
    #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname
    end#1\endcsname
  \renewenvironment{#1}%
  {\linenomath\csname old#1\endcsname}%
  {\csname oldend#1\endcsname\endlinenomath}%
}
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}%
}
\patchBothAmsMathEnvironmentsForLineno{equation}
\patchBothAmsMathEnvironmentsForLineno{align}
\patchBothAmsMathEnvironmentsForLineno{flalign}
\patchBothAmsMathEnvironmentsForLineno{alignat}
\patchBothAmsMathEnvironmentsForLineno{gather}
\patchBothAmsMathEnvironmentsForLineno{multline}


==> preamble/preamble_math.tex <==
% !TEX root = main.tex


\usepackage{centernot}

\DeclareRobustCommand{\mb}[1]{\ensuremath{\mathbf{\boldsymbol{#1}}}}
% \DeclareRobustCommand{\mb}[1]{\mathbold{#1}}

\DeclareRobustCommand{\KL}[2]{\ensuremath{\textrm{KL}\left(#1\;\|\;#2\right)}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\crefname{lemma}{lemma}{lemmas}
\Crefname{lemma}{Lemma}{Lemmas}
\crefname{thm}{theorem}{theorems}
\Crefname{thm}{Theorem}{Theorems}
\crefname{prop}{proposition}{propositions}
\Crefname{prop}{Proposition}{Propositions}
\crefname{defn}{definition}{definitions}
\Crefname{defn}{Definition}{Definitions}
\creflabelformat{equation}{#1#2#3}
\crefname{equation}{eq.}{eqs.}
\Crefname{equation}{Eq.}{Eqs.}
\Crefname{section}{\S}{\S}
\crefname{figure}{fig.}{figs.}
\Crefname{figure}{Fig.}{Figs.}
\crefname{algorithm}{alg.}{algs.}
\Crefname{algorithm}{Alg.}{Algs.}


\newtheorem{thm}{Theorem} % reset theorem numbering for each chapter
\newtheorem{defn}{Definition} % definition numbers are dependent on theorem numbers
\newtheorem{prop}[thm]{Proposition}
\newtheorem{exmp}[thm]{Example} % same for example numbers
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{assumption}[thm]{Assumption}
\newtheorem{corollary}[thm]{Corollary}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\renewcommand{\mid}{~\vert~}
\newcommand{\prm}{\:;\:}

\newcommand{\mbw}{\mb{w}}
\newcommand{\mbW}{\mb{W}}

\newcommand{\mbx}{\mb{x}}
\newcommand{\mbX}{\mb{X}}

\newcommand{\mby}{\mb{y}}
\newcommand{\mbY}{\mb{Y}}

\newcommand{\mbz}{\mb{z}}
\newcommand{\mbZ}{\mb{Z}}
\newcommand{\mbT}{\mb{T}}
\newcommand{\mbA}{\mb{A}}
\newcommand{\mba}{\mb{a}}

\newcommand{\mbI}{\mb{I}}
\newcommand{\mbone}{\mb{1}}

\newcommand{\mbL}{\mb{L}}

\newcommand{\mbtheta}{\mb{\theta}}
\newcommand{\mbTheta}{\mb{\Theta}}
\newcommand{\mbomega}{\mb{\omega}}
\newcommand{\mbOmega}{\mb{\Omega}}
\newcommand{\mbsigma}{\mb{\sigma}}
\newcommand{\mbSigma}{\mb{\Sigma}}
\newcommand{\mbphi}{\mb{\phi}}
\newcommand{\mbPhi}{\mb{\Phi}}

\newcommand{\mbalpha}{\mb{\alpha}}
\newcommand{\mbbeta}{\mb{\beta}}
\newcommand{\mbgamma}{\mb{\gamma}}
\newcommand{\mbeta}{\mb{\eta}}
\newcommand{\mbmu}{\mb{\mu}}
\newcommand{\mbrho}{\mb{\rho}}
\newcommand{\mblambda}{\mb{\lambda}}
\newcommand{\mbzeta}{\mb{\zeta}}

\newcommand\dif{\mathop{}\!\mathrm{d}}
\newcommand{\diag}{\textrm{diag}}
\newcommand{\supp}{\textrm{supp}}

\newcommand{\V}{\mathbb{V}}
\newcommand{\bbH}{\mathbb{H}}

\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}

\newcommand{\cL}{\mathcal{L}}
\newcommand{\cD}{\mathcal{D}}

\newcommand{\cN}{\mathcal{N}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\Gam}{\textrm{Gam}}
\newcommand{\InvGam}{\textrm{InvGam}}

% \newcommand{\qedsymbol}{\rule{0.7em}{0.7em}}

\newcommand{\g}{\, | \,}
\newcommand{\s}{\, ; \,}

\newcommand{\indpt}{\protect\mathpalette{\protect\independenT}{\perp}}
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 


\usepackage{booktabs,arydshln}
\makeatletter
\def\adl@drawiv#1#2#3{%
        \hskip.5\tabcolsep
        \xleaders#3{#2.5\@tempdimb #1{1}#2.5\@tempdimb}%
                #2\z@ plus1fil minus1fil\relax
        \hskip.5\tabcolsep}
\newcommand{\cdashlinelr}[1]{%
  \noalign{\vskip\aboverulesep
           \global\let\@dashdrawstore\adl@draw
           \global\let\adl@draw\adl@drawiv}
  \cdashline{#1}
  \noalign{\global\let\adl@draw\@dashdrawstore
           \vskip\belowrulesep}}
\makeatother

\newenvironment{proofsk}{%
  \renewcommand{\proofname}{Proof sketch}\proof}{\endproof}


==> preamble/preamble_tikz.tex <==
% !TEX root = main.tex

\usepackage{tikz}
\usetikzlibrary{bayesnet}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\pgfplotsset{plot coordinates/math parser=false}
\usepgfplotslibrary{statistics}

\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{edgelayer,nodelayer,main}

\definecolor{hexcolor0xbfbfbf}{rgb}{0.749,0.749,0.749}

\tikzset{>=latex}
\tikzstyle{none}   = [inner sep=0pt]
\tikzstyle{line}   = [ thick, -, shorten <=1pt, shorten >=1pt ]
\tikzstyle{arrow}  = [ thick,  ->, shorten <=1pt, shorten >=1pt ]
\tikzstyle{ardash} = [ thick dotted, ->, shorten <=1pt, shorten >=1pt ]

\tikzstyle{empty}=[circle,opacity=0.0,text opacity=1.0,minimum width=4pt,minimum height=4pt]
\tikzstyle{box}=[rectangle,fill=White,draw=Black]
\tikzstyle{filled}=[circle,fill=hexcolor0xbfbfbf,draw=Black]
\tikzstyle{hollow}=[circle,fill=White,draw=Black]
\tikzstyle{param}=[rectangle,fill=Black,draw=Black,inner sep=0pt,minimum width=4pt,minimum height=4pt]
\tikzstyle{paramhollow}=[rectangle,fill=White,draw=Black,inner sep=0pt,minimum
width=4pt,minimum height=4pt]

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

==> table/fairres.tex <==
% !TEX root = ../fair_dcf.tex
%
%\begin{table*}
%	\footnotesize
%	\begin{center}
%		\begin{tabular}{lcccp{1cm}ccc} 
%			\toprule
%			& \multicolumn{3}{c}{\textbf{\gls{EO} Metric ($\times 10^-2$)}} && \multicolumn{3}{c}{\textbf{\gls{AA} Metric ($\times 10^-2$)}}\\
%			\midrule
%			& \textbf{Adult} & \textbf{COMPAS}  & \textbf{German Credit} && \textbf{Adult} & \textbf{COMPAS}  & \textbf{German Credit}\\
%			\midrule
%			ML predictor $f_\ML$ &2.5(1.9)&-68.1(42.1)&-5.4(2.5) && 16.2(12.0) & -104.9(59.7) & -3.9(1.8)\\
%			\cdashlinelr{1-6}
%			\glsreset{FTU}\gls{FTU} &\textbf{0(0)}&\textbf{0(0)}&\textbf{0(0)} & & & & \\
%			\gls{EO} predictor $f_\eo$ &\textbf{0(0)}&\textbf{0(0)}&\textbf{0(0)} & & & & \\
%			\cdashlinelr{1-6}
%			FairLearning \citep{kusner2017counterfactual} &-14.8(9.1)&-41.2(29.4)&-1.4(0.7) & &\textbf{0(0)}&\textbf{0(0)}&\textbf{0(0)} \\
%			\gls{AA} predictor $f_\rmaa$ &-9.1(9.8)&-41.2(29.4)&-1.3(0.6) & &\textbf{0(0)}&\textbf{0(0)}&\textbf{0(0)} \\
%			% \gls{AA} predictor $f_\rmaa$ w/o $S$ &&&\\
%			\bottomrule
%		\end{tabular}
%		\caption{Both \gls{EO} predictor $f_\eo$ and unaware ML achieve zero in the \gls{EO} metric; they satisfy the \gls{EO} target. (Lower is
%			better.) Differences in counterfactual prediction when we intervene on the sensitive attribute while holding others fixed.\label{tab:cfdiffgivA}}
%	\end{center}
%	% \vspace{-10pt}
%\end{table*}


\begin{table}
	\footnotesize
%	\begin{center}
		
		\begin{tabular}{lccc} 
			\toprule
			&\multicolumn{3}{c}{\textbf{\gls{EO} Metric ($\times 10^-2$)}} \\
			\midrule
			&\textbf{Adult} & \textbf{COMPAS} & \textbf{Credit}\\
			\midrule
			ML predictor $f_\ML$ & 2.5 & -68.1 &-5.4 \\
			\cdashlinelr{1-4}
			\gls{FTU} & \textbf{0} & \textbf{0} & \textbf{0}\\
			\gls{EO} predictor $f_\eo$ & \textbf{0} & \textbf{0} & \textbf{0}\\
			\cdashlinelr{1-4}
			FairLearning  & -14.8 & -41.2 & -1.4\\
			\gls{AA} predictor $f_\rmaa$ & -9.1 & 41.2 & -1.3 \\
			% \gls{AA} predictor $f_\rmaa$ w/o $S$ &&&\\
			\bottomrule
		\end{tabular}
		\caption{Both \gls{EO} predictor $f_\eo$ and unaware ML are \gls{EO}-fair; they achieve zero in the \gls{EO} metric (lower is
			better.) ML predictor $f_\ML$, FairLearning \cite{kusner2017counterfactual} and \gls{AA} predictor $f_\rmaa$ 
			are not fair in \gls{EO}.
			Mean \gls{EO} metric ($\times 10^-2$) across individuals; standard deviation is $\leq 0.42$.
%			Differences in counterfactual prediction when we intervene on the sensitive attribute while holding others fixed.
			\label{tab:cfdiffgivA}}
%	\end{center}
	% \vspace{-10pt}
\end{table}


\begin{table}
	\footnotesize
%	\begin{center}
		\begin{tabular}{lccc} 
			\toprule
			&\multicolumn{3}{c}{\textbf{\gls{AA} Metric ($\times 10^-2$)}} \\
			\midrule
			&\textbf{Adult} & \textbf{COMPAS} & \textbf{Credit}\\
			\midrule
			ML predictor $f_\ML$ &16.2 & -104.9 & -3.9\\
			\cdashlinelr{1-4}
			\gls{FTU} & 14.8 &-52.9 & -2.0\\
			% \cdashlinelr{1-6}
			\gls{EO} predictor $f_\eo$ & 14.1  &-36.8 & 1.5 \\
			\cdashlinelr{1-4}
			FairLearning  & \textbf{0} & \textbf{0} & \textbf{0} \\
			\gls{AA} predictor $f_\rmaa$ & \textbf{0} & \textbf{0} & \textbf{0} \\
			% \gls{AA} predictor $f_\rmaa$ w/o $S$ &&&\\
			\bottomrule
		\end{tabular}
		\caption{\gls{AA} predictor $f_\rmaa$ and FairLearning \citep{kusner2017counterfactual} are \gls{AA}-fair; they achieve zero in the \gls{AA} metric (lower is
			better). 
			Mean \gls{AA} metric ($\times 10^-2$) across individuals; 
			standard deviation is $\leq 0.59$.)\label{tab:cfdiff}}
%	\end{center}
	% \vspace{-10pt}
\end{table}


\begin{table}
	\footnotesize
	\begin{center}
		\begin{tabular}{lccc} 
			\toprule
			&\multicolumn{3}{c}{\textbf{Symmetric \gls{KL}($\times 10^-2$)}} \\
			\midrule
			&\textbf{Adult} & \textbf{COMPAS} & \textbf{Credit}\\
			\midrule
			ML predictor $f_\ML$ &15.0 & 17.1 & 18.6\\
			\cdashlinelr{1-4}
			\gls{FTU} &0.122 &0.005&0.156\\
			% \cdashlinelr{1-6}
			\gls{EO} predictor $f_\eo$ &0.126&0.005&0.132\\
			\cdashlinelr{1-4}
			FairLearning  &5.3 &\textbf{0.2} & 8.3\\       
			\gls{AA} predictor $f_\rmaa$ &\textbf{1.5}&\textbf{0.2}&\textbf{7.8}\\
			% \gls{AA} predictor $f_\rmaa$ w/o $S$ &&&\\
			\bottomrule
		\end{tabular}
		\caption{The \gls{AA} predictor $f_\rmaa$ has close-to-zero
			\gls{KL} divergence in prediction distributions; it
			achieves demographic parity. (Lower is better.)
			\label{tab:symmkl}}
	\end{center}
	% \vspace{-10pt}
\end{table}




%\begin{table*}
%\footnotesize
%  \begin{center}
%    \begin{tabular}{lrrrrrrrrr} 
%     \toprule
%      &\multicolumn{1}{c}{\textbf{Adult}} &&\multicolumn{1}{c}{\textbf{COMPAS}} &&\multicolumn{1}{c}{\textbf{German Credit}} \\
%     \midrule
%      ML predictor $f_\ML$ &0.025(0.019)&&-0.681(0.421)&&-0.054(0.025)\\
%      \cdashlinelr{1-6}
%      \glsreset{FTU}\gls{FTU} &\textbf{0.000(0.000)}&&\textbf{0.000(0.000)}&&\textbf{0.000(0.000)}\\
%      \gls{EO} predictor $f_\eo$ &\textbf{0.000(0.000)}&&\textbf{0.000(0.000)}&&\textbf{0.000(0.000)}\\
%      \cdashlinelr{1-6}
%      FairLearning \citep{kusner2017counterfactual} &-0.148(0.091)&&-0.412(0.294)&&-0.014(0.007)\\
%      \gls{AA} predictor $f_\rmaa$ &-0.091(0.098)&&-0.412(0.294)&&-0.013(0.006)\\
%      % \gls{AA} predictor $f_\rmaa$ w/o $S$ &&&\\
%      \bottomrule
%    \end{tabular}
%    \caption{Both \gls{EO} predictor $f_\eo$ and unaware ML achieve zero in the \gls{EO} metric; they satisfy the \gls{EO} target. (Lower is
%    better.) Differences in counterfactual prediction when we intervene on the sensitive attribute while holding others fixed.\label{tab:cfdiffgivA}}
%  \end{center}
%  % \vspace{-10pt}
%\end{table*}


%\begin{table*}
%	\footnotesize
%	\begin{center}
%		\begin{tabular}{lrrrrrrrrr} 
%			\toprule
%			&\multicolumn{1}{c}{\textbf{Adult}} &&\multicolumn{1}{c}{\textbf{COMPAS}} &&\multicolumn{1}{c}{\textbf{German Credit}} \\
%			\midrule
%			ML predictor $f_\ML$ &0.162(0.120)&&-1.049(0.597)&&-0.039(0.018)\\
%			\cdashlinelr{1-6}
%			\glsreset{FTU}\gls{FTU} &0.148(0.117)&&-0.529(0.301)&& -0.020(0.010)\\
%			% \cdashlinelr{1-6}
%			\gls{EO} predictor $f_\eo$ &0.141(0.103)&&-0.368(0.212)&&0.015(0.007)\\
%			\cdashlinelr{1-6}
%			FairLearning \citep{kusner2017counterfactual} &\textbf{0.000(0.000)}&&\textbf{0.000(0.000)}&&\textbf{0.000(0.000)}\\
%			\gls{AA} predictor $f_\rmaa$ &\textbf{0.000(0.000)}&&\textbf{0.000(0.000)}&&\textbf{0.000(0.000)}\\
%			% \gls{AA} predictor $f_\rmaa$ w/o $S$ &&&\\
%			\bottomrule
%		\end{tabular}
%		\caption{\gls{AA} predictor $f_\rmaa$ achieves zero in the \gls{AA} metric; it is counterfactually fair. (Lower is
%			better. Differences in counterfactual predictions when intervening on the sensitive attribute and allow
%			other attributes to change correspondingly.)\label{tab:cfdiff}}
%	\end{center}
%	% \vspace{-10pt}
%\end{table*}
%
%
%\begin{table*}
%\footnotesize
%  \begin{center}
%    \begin{tabular}{lrrrrrrrrr} 
%     \toprule
%      &\multicolumn{1}{c}{\textbf{Adult}} &&\multicolumn{1}{c}{\textbf{COMPAS}} &&\multicolumn{1}{c}{\textbf{German Credit}} \\
%     \midrule
%      ML predictor $f_\ML$ &0.150&&0.171&&0.186\\
%      \cdashlinelr{1-6}
%      \glsreset{FTU}\gls{FTU} &0.122&&0.005&&0.156\\
%      % \cdashlinelr{1-6}
%      \gls{EO} predictor $f_\eo$ &0.126&&0.005&&0.132\\
%      \cdashlinelr{1-6}
%      FairLearning \citep{kusner2017counterfactual} &0.053&&\textbf{0.002}&&0.083\\       \gls{AA} predictor $f_\rmaa$ &\textbf{0.015}&&\textbf{0.002}&&\textbf{0.078}\\
%      % \gls{AA} predictor $f_\rmaa$ w/o $S$ &&&\\
%      \bottomrule
%    \end{tabular}
%    \caption{ \gls{AA} predictor $f_\rmaa$ has close-to-zero \gls{KL}
%    divergence in prediction distributions; it achieves demographic
%    parity. (Lower is better.) \label{tab:symmkl}}
%  \end{center}
%  % \vspace{-10pt}
%\end{table*}






==> table/prediction.tex <==
% !TEX root = ../fair_dcf.tex

\begin{table}
	\footnotesize
	\begin{center}
		\begin{tabular}{lccc} 
			\toprule
			\multicolumn{3}{c}{\textbf{Prediction Score ($\times 10^{-2}$)}}\\
			&\textbf{Adult} & \textbf{COMPAS} & \textbf{Credit}\\
			\midrule
			ML predictor $f_\ML$ & 78.6 & 28.0 & 64.7\\
			\cdashlinelr{1-4}
			\gls{FTU} & 77.3 &\textbf{25.6}& 63.4\\
			% \cdashlinelr{1-6}
			\gls{EO} predictor $f_\eo$ &\textbf{77.4}&\textbf{25.6}&\textbf{64.5}\\
			\cdashlinelr{1-4}
			FairLearning &75.1&\textbf{22.7}&63.5\\
			\gls{AA} predictor $f_\rmaa$  &\textbf{77.1}&\textbf{22.7}&\textbf{64.3}\\
			% \gls{AA} predictor $f_\rmaa$ w/o $S$ &0.779&0.176&\\
			\bottomrule
		\end{tabular}
		\caption{ML predictor $f_\ML$ always produces the best
			prediction scores. \gls{EO} predictor $f_\eo$ predicts the best among the
			fair predictors. The prediction score is mean accuracy with binary
			outcomes. For real-valued outcomes, it is the coefficient of
			determination $R^2$ of the prediction. (Higher is better.)
			\label{tab:prediction}}
	\end{center}
	% \vspace{-10pt}
\end{table}

%\begin{table*}
%\footnotesize
%  \begin{center}
%    \begin{tabular}{lccccccccc} 
%     \toprule
%      &\multicolumn{1}{c}{\textbf{Adult}} & &\multicolumn{1}{c}{\textbf{COMPAS}} & & \multicolumn{1}{c}{\textbf{German Credit}} \\
%     \midrule
%      ML predictor $f_\ML$ &0.786&&0.280&&0.647\\
%      \cdashlinelr{1-6}
%      \glsreset{FTU}\gls{FTU} &0.773&&\textbf{0.256}&&0.634\\
%      % \cdashlinelr{1-6}
%      \gls{EO} predictor $f_\eo$ (this paper) &\textbf{0.774}&&\textbf{0.256}&&\textbf{0.645}\\
%      \cdashlinelr{1-6}
%      FairLearning \citep{kusner2017counterfactual} &0.751&&\textbf{0.227}&&0.635\\
%      \gls{AA} predictor $f_\rmaa$ (this paper) &\textbf{0.771}&&\textbf{0.227}&&\textbf{0.643}\\
%      % \gls{AA} predictor $f_\rmaa$ w/o $S$ &0.779&0.176&\\
%      \bottomrule
%    \end{tabular}
%    \caption{Prediction scores. ML predictor $f_\ML$ always produces the best
%    predictions. \gls{EO} predictor $f_\eo$ predicts the best among the
%    fair predictors. The prediction score is mean accuracy with binary
%    outcomes. For real-valued outcomes, it is the coefficient of
%    determination $R^2$ of the prediction. (Higher is better.)
%    \label{tab:prediction}}
%  \end{center}
%  % \vspace{-10pt}
%\end{table*}
%

